Privacy-Preserving Image Classification in the Local Setting

Image data has been greatly produced by individuals and commercial vendors in the daily life, and it has been used across various domains, like advertising, medical and traffic analysis. Recently, image data also appears to be greatly important in social utility, like emergency response. However, the privacy concern becomes the biggest obstacle that prevents further exploration of image data, due to that the image could reveal sensitive information, like the personal identity and locations. The recent developed Local Differential Privacy (LDP) brings us a promising solution, which allows the data owners to randomly perturb their input to provide the plausible deniability of the data before releasing. In this paper, we consider a two-party image classification problem, in which data owners hold the image and the untrustworthy data user would like to fit a machine learning model with these images as input. To protect the image privacy, we propose to locally perturb the image representation before revealing to the data user. Subsequently, we analyze how the perturbation satisfies {\epsilon}-LDP and affect the data utility regarding count-based and distance-based machine learning algorithm, and propose a supervised image feature extractor, DCAConv, which produces an image representation with scalable domain size. Our experiments show that DCAConv could maintain a high data utility while preserving the privacy regarding multiple image benchmark datasets.

==> manuscript/sections/experiment2.tex <==
\section{Experiment}
We evaluate DCAConv over three popular benchmark image datasets, the MNIST, Fashion-MNIST\footnote{https://github.com/zalandoresearch/fashion-mnist}, YaleB\footnote{vision.ucsd.edu/~iskwak/ExtYaleDatabase/ExtYaleB.html}.

\iffalse
and BioID\footnote{https://ftp.uni-erlangen.de/pub/facedb/readme.html} facial dataset.
\fi
\textbf{The MNIST dataset} contains $28 \times 28$ grayscale images of handwritten digits that from 0 to 9, in which there are 60,000 samples for training and 10,000 samples for testing.

\textbf{The Fashion-MNIST dataset} contains the grayscale article images that each sample associates with a label from 10 classes. The dataset is intended to replace the overused MNIST dataset, and shares the same image size and structure of training and testing splits.

\textbf{The YaleB face dataset} contains grayscale photos of 27 subjects and each subject has around 600 samples in average, we select samples based on the light condition and the head position, which results in around 250 samples per subject. The face is extracted and scaled to 70 $\times$ 70.


To study the utility and privacy trade-off in terms of the domain size $d$ and privacy parameter $\epsilon$, DCAConv is used to produce the output with various domain sizes and is compared to three other image representations, e.g. raw pixel, Histogram of Oriented Gradients (HOG) and Binarized Neural Network (BNN)\cite{courbariaux2016binarized}. Here we briefly introduce each representation below:

\textbf{DCAConv} The details of DCAConv is presented in previous section, and there are two convolution layers used in the experiments, where the output domain size $d$ is determined by $L_2$, $d = 2^{L_2}$.

\textbf{Pixel} The grayscale representation of the image, where the original value of each pixel is between [0,255]. To make a fair comparison, the original pixel is downscaled to have the same size as the DCAConv output domain. For example, the pixel is downscaled to [0,15] using a MinMaxScaler\footnote{http://scikit-learn.org/stable/modules/generated/\\sklearn.preprocessing.MinMaxScaler.html} to match the DCAConv with 4 $L_2$ filters.

\textbf{HOG} The descriptor provides the histograms of directions of gradients that are used to capture the edges and corners of an image, which results in a fixed length of floating vector. Conventionally, the histograms are contrast-normalized to improve the accuracy. Instead of directly adopting the normalized histogram, a Bag of Visual Words (BOVW) model is further associated with the HOG descriptors. More specifically, the K-Means clustering is performed over the generated descriptors and the center of each cluster is used as the visual dictionary’s vocabularies. Finally, the frequency histogram is made from the visual vocabularies and is served as BOVW. Unlike DCAConv, the domain size of the BOVW is fixed once the number of clusters is determined and there is no significant difference observed after tuning the number of clusters in our experiment.

\textbf{BNN} As we mention early, the reason that it is hard to apply randomized response to CNN is that the data flow is continuous. However, there are studies to replace the weights and activation with discrete values for the purpose of improving the power-efficiency. BNN is one of such research work, which modifies the convolution layer and activation function, to transform the data flow from the floating number to $\{+1,-1\}$. For the implementation of BNN, we take the suggested values for parameters like the number of hidden units in the fully connected layer, but with the same number of convolution layer and filters as DCAConv. Once the training of BNN is finished, we take the activated binarized output before the fully connected layer and perturb it.


Regarding all four representations, randomized response is applied to each one with different values of privacy parameter $\epsilon$ and the perturbed inputs are then used to fit the Naive Bayes and KNN classifiers. The classification result confirms our analysis with respect to the relationship between the domain size and $\epsilon$, it also demonstrates the effectiveness of the DCAConv over other image representations. All experiments are repeated 10 times, the mean and standard deviation of the classification accuracy are drawn in figures. 
\begin{figure*}[ht!]
\centering
\begin{subfigure}[t]{1\textwidth}
\begin{subfigure}[t]{.32\textwidth}
\centering
\includegraphics[width=1\textwidth]{./exp/nb_Fashion-MNIST}
\caption{Fashion-MNIST}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
\centering
\includegraphics[width=1\textwidth]{./exp/nb_MNIST}
\caption{MNIST}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
\centering
\includegraphics[width=1\textwidth]{./exp/nb_YaleB}
\caption{YaleB}
\end{subfigure}
\end{subfigure}
%\includegraphics[width=.32\textwidth]{effic_Aloi}\quad
%\includegraphics[width=.32\textwidth]{effic_Facebook}\quad
%\includegraphics[width=.32\textwidth]{effic_MillionSong}
\medskip
\caption{Comparison of DCAConv, Pixel, BOVW and BNN in terms of Naive Bayes classification. DCAConv hyper-parameters, filter size: 7$\times$7, filter stride size: 1$\times$1, $L_1$:5, $L_2$:4, pooling window size: 2$\times$2, pooling stride size: 1$\times$1. BOVW is represented with 200 vocabularies.}
\label{fig:nb}
\end{figure*}
\subsection{Naive Bayes}

We first show the Naive Bayes classification accuracy with all four image representations. Fig.~\ref{fig:nb} displays the result regarding three datasets, for each subfigure, the horizontal axis specifies $\epsilon$ for each individual feature, and the vertical axis shows the classification accuracy. In the experiment, two domain sizes of DCAConv is examined, e.g. $d=16$ and $d=2$, and Pixel representation is also downscaled to 16. For the information loss caused by the downscaling, we don't observe a significant degrading in terms of the classification accuracy. From the figure, for all three datasets, the classifier performs no better than the random guessing when $\epsilon = 0.001$, which implies a severe utility damage in the high privacy regime. For both MNIST and Fashion-MNIST, the accuracy of DCAConv increases as $\epsilon \geq 0.01$, and it shows that the representation with a small domain size ($d=2$) performs better than the large one ($d=16$), the pattern continues tills $\epsilon=0.1$. As $\epsilon$ grows, the perturbation becomes less and the representation of DCAConv with a large domain size keeps improving the accuracy due to more information carried than the small domain. For YaleB, the similar pattern delays to a relatively large $\epsilon$ due to the hardness of Naive Bayes regarding the facial dataset. Table ~\ref{tab:dcaconv_nb} provides the Naive Bayes accuracy of DCAConv when $\epsilon \geq 0.1$, where the last column gives the ground truth as no randomized response applied. From the table, it can be seen that DCAConv (d=2) quickly converges to the ground truth from $\epsilon=0.5$. 
Finally, the figure also shows that DCAConv achieves either higher or compatible accuracy given the same domain size, e.g. DCAConv (d=16) vs. Pixel (d=16), DCAConv (d=2) vs. BNN. And among all representations, BOVW suffers from the lowest accuracy due to the large domain size for each $\epsilon$.


\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \diagbox{dataset}{$\epsilon$}      & 0.1            & 0.5            & 1.0            & 1.5            & 2.0            & 2.5            & 3.0            & 3.5            & 4.0            & $\infty$ \\ \hline
\multirow{3}{*}{$d=2$} & MNIST         & 76.38 & 77.30 & 77.21 & 77.10 & 77.04 & 76.96 & 76.91 & 76.89 & 76.83 & 76.60 \\ \cline{2-12} 
                             & Fashion-MNIST & 58.96 & 68.27 & 68.71 & 68.88 & 68.89 & 68.94 & 68.94 & 68.90 & 68.90 & 68.80 \\ \cline{2-12} 
                             & YaleB         &  12.01     &   34.76    &  33.94     &  38.38     & 43.16       &   42.91    &   42.86    &  42.74     &  42.74     & 42.74      \\ \hline

\multirow{3}{*}{$d=16$} & MNIST         & 77.52 & 86.35 & 87.15 & 87.19 & 87.07 & 86.97 & 86.92 & 86.92 & 86.90 & 86.90 \\ \cline{2-12} 
                             & Fashion-MNIST & 58.96 & 68.27 & 68.71 & 68.88 & 68.89 & 68.94 & 68.94 & 68.90 & 68.90 & 68.80 \\ \cline{2-12} 
                             & YaleB &  10.52 &   44.27    &  70.29     &  71.32     & 78.89       &  79.43     &  80.63     &  80.70    &   81.32    &  81.71  \\ \hline

\end{tabular}
\caption{Naive Bayes Classification accuracy ($\%$) with DCAConv. The last column provides the ground truth as no randomized response applied. Due to the space limit, the standard deviation of the measured accuracy is omitted here.}
\label{tab:dcaconv_nb}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \diagbox{dataset}{$\epsilon$}      & 0.1            & 0.5            & 1.0            & \textbf{1.5}            & 2.0            & 2.5            & \textbf{3.0}            & 3.5            & 4.0            & $\infty$\\ \hline
\multirow{3}{*}{$d=2$}   & MNIST         &  65.96               &    85.25            &   88.27             &    \textbf{89.21}            &   89.69             &    89.95            &    90.04            &    90.19            & 90.24                &  90.20  \\ \cline{2-12} 
                       & Fashion-MNIST         & 69.66  & 70.90 & 70.62 & \textbf{70.52} & 70.43 & 70.39 & 70.39 & 70.37 & 70.32 & 70.30 \\ \cline{2-12} 
                       & YaleB & 79.33 & 95.50 & 95.35 & \textbf{95.46} & 95.58 & 95.55 & 95.61 &    95.66 & 95.75 & 95.80 \\ \hline
\multirow{3}{*}{$d=16$}   & MNIST  & 24.72  & 68.92 & 81.96 & 86.05 & 88.00 & 89.37 & \textbf{89.95} &90.27 & 90.46 &  90.50 \\ \cline{2-12} 
                       & Fashion-MNIST  & 20.56 & 48.58 & 57.35 & 63.40 & 68.21 & 71.54 & \textbf{74.14} & 75.64 & 76.73 & 78.70 \\ \cline{2-12} 
                       & YaleB & 6.01  & 49.56  & 90.76 & 95.18 & 95.88 & 95.91 & \textbf{95.88} & 95.77 & 95.77 & 95.92 \\ \hline

\end{tabular}
\caption{KNN Classification accuracy ($\%$) with DCAConv,  where $ln(16+1) \approx 2.83$ and $ln(2+1) \approx 1.10$. The last column provides the ground truth as no randomized response applied. Due to the space limit, the standard deviation of the measured accuracy is omitted here.}
\label{tab:dcaconv_knn}
\end{table*}


\subsection{KNN}
\begin{figure*}[ht!]
\centering
\begin{subfigure}[t]{1\textwidth}
\begin{subfigure}[t]{.32\textwidth}
\centering
\includegraphics[width=1\textwidth]{./exp/knn_Fashion-MNIST}
\caption{Fashion-MNIST}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
\centering
\includegraphics[width=1\textwidth]{./exp/knn_MNIST}
\caption{MNIST}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
\centering
\includegraphics[width=1\textwidth]{./exp/knn_YaleB}
\caption{YaleB}
\end{subfigure}
\end{subfigure}
%\includegraphics[width=.32\textwidth]{effic_Aloi}\quad
%\includegraphics[width=.32\textwidth]{effic_Facebook}\quad
%\includegraphics[width=.32\textwidth]{effic_MillionSong}
\medskip
\caption{Comparison of DCAConv, Pixel, BOVW and BNN in terms of KNN classification. DCAConv hyper-parameters, filter size: 7$\times$7, filter stride size: 1$\times$1, $L_1$:5, $L_2$:4, pooling window size: 2$\times$2, pooling stride size: 1$\times$1. BOVW is represented with 200 vocabularies.}
\label{fig:knn}
\end{figure*}
The perturbed input is used to fit the KNN classifier as well, and the result is shown in Fig~\ref{fig:knn}, where the vertical axis specifies the classification accuracy. When $\epsilon \leq 0.01$, for all representations, the classifier performs no better than the random guessing. As $\epsilon$ grows, the classifications with DCAConv (d=2) and BNN quickly show utility gain. As analyzed in Section III, the probability of being the true $\ell_2$ distance is bigger than $\frac{1}{2}$ as $\epsilon \geq ln(d+1)$. To further illustrate the point, Table ~\ref{tab:dcaconv_knn} presents the KNN accuracy of DCAConv when $\epsilon \geq 0.1$, it can be seen that the accuracy of DCAConv(d=2) almost matches the ground truth regarding all three datasets (corresponding accuracies are in bold) when $\epsilon \geq 1.5$ . Furthermore, the accuracy of DCAConv (d=16) is within $5\%$ of the ground truth as $\epsilon \geq 3.0$. Other representations, e.g. Pixel and BOVW also confirm our KNN classifier utility analysis in terms of $d$ and $\epsilon$. Additionally, the accuracy result also shows that DCAConv performs either better or compatible under the same domain size. 

\subsection{Naive Bayes vs. KNN}
Our experimental evaluation gives the classification result with respect to Naive Bayes and KNN classifiers. Comparison between both classifiers shows that Naive Bayes can provide a good utility under a high privacy (small $\epsilon$) constraint, where it may due to that the noise is eliminated by the frequency estimator. Unlike Naive Bayes, the utility of KNN is determined by the probability of preserving the true proximity between the perturbed training data and testing data, where we argue that the probability is bigger than $\frac{1}{2}$ as $\epsilon \geq ln(d+1)$, which implies that KNN could maintain a good utility in a low privacy (large $\epsilon$) regime.




==> manuscript/sections/utilityAnalysis_nb_knn.tex <==
\section{Problem Definition and Solution Analysis}
\subsection{Problem Definition}
\begin{figure}
  \centering
    \includegraphics[width=0.5\textwidth]{./researchProblem/problem2}
  \caption{Problem Overview. An image held by Data Owner $O_i$ is represented as a vector $x_i = \{x_{i1},x_{i2},\dots,x_{im}\}, x_{ij} \in [d]$, each vector associates with a label $y_i$, the Data User would like to fit a classifier with such vectors from all $n$ Data Owners. To protect the privacy of $x_i$, a perturbation is required to satisfy $\epsilon_j$-LDP for the $j$th feature.}
  \label{fig:problem}
\end{figure}
As Fig.\ref{fig:problem} shows, in this paper, we consider the following problem: \textit{Given $n$ Data Owners, each Data Owner $O_i$ holds a set of images that are represented as a $m$-dimensional feature vectors. For ease of analysis, here it is assume that only one image is possessed by $O_i$ and it is denoted as $x_i = \{x_{i1},x_{i2},\dots,x_{im}\}, x_{ij} \in [d]$. Each image $x_i$  associates with a label $y_i$, for instance, the images held by each data owner is about the handwritten digit, and $y_i$ indicates the corresponding digit of $x_i$; the untrustworthy Data User would like to fit an image classifier with $x_i,y_i, i\in \{1,2,\dots,n\}$ as input while satisfying $\epsilon_j$-LDP for the $j$th feature of $x_i$}. It should be noted that the images held by each data owner are perturbed independently, so there are no difference to perturb a set of images or a single image at $O_i$. With respect to image classification, the effectiveness of both Naive Bayes and KNN classifiers have been demonstrated through previous work\cite{boiman2008defense,mccann2012local}, which are studied in this work.

For the threat model, the adversary is intended to learn individual image $x_i$, who could be either the untrustworthy data user, a participating data owner or an outside attacker. It assumes that adversaries might have arbitrary background knowledge and there might be a collusion among them. The goal is maintain the data utility in terms of image classification while protecting the data privacy.

\subsection{Input Perturbation}

In this paper, we mainly investigate to use Randomized Response to satisfy $\epsilon_{ij}$-LDP for $x_{ij}$, which is perturbed independently. Given a $x_i,y_i$, we further assume that $x_i'$ is the vector after perturbation and the class label $y_{i}\in \{C_{1}, C_{2}, \dots, C_{k}\}$. Firstly, we show how to build the Naive Bayes classifier by leveraging the aggregation result of the perturbed input.

\subsubsection{Naive Bayes Classifier}
Naive Bayes classifier refers to the ``probabilistic classifier'' based on the Bayes' theorem, given a testing sample $x_t$, the probability that it is classified as $C_k$ is given by:
\begin{align}
Pr[C_k|x_t] & = \frac{Pr[C_k]Pr[x_t|C_k]}{Pr[x_t]} \\ 
& = \frac{Pr[C_k]Pr[x_{t1},x_{t2},\dots,x_{tm}|C_k]}{Pr[x_{t1},x_{t2},\dots,x_{tm}]}
\end{align}
The ``Naive'' assumes that assume that each feature $x_{ti}$ is conditionally independent of every other feature $x_{tj},i\neq j$, given the class $C_k$ , which implies: 
\begin{equation}
Pr[x_{tj}|C_k,x_{t1},x_{t2},\dots,x_{t(j-1)},x_{t(j+1)},\dots,x_{tm}] = Pr[x_{tj}|C_k]
\end{equation}
$Pr[C_k|x_t]$ becomes:
\begin{equation}
Pr[C_k|x_t] = \frac{Pr[C_k]\prod_{j=1}^mPr[x_{tj}|C_k]}{Pr[x_{t1},x_{t2},\dots,x_{tm}]}
\end{equation}
Since the evidence $Pr[x_{t1},x_{t2},\dots,x_{tm}]$ is constant, thus:
\begin{equation}
Pr[C_k|x_t] \propto Pr[C_k]\prod_{j=1}^mPr[x_{tj}|C_k]
\end{equation}

With the decision rule of \textit{maximum a posteriori}, the predicted class is given by:

\begin{equation}
\hat{C} = \argmax_{C_k} Pr[C_k]\prod_{j=1}^mPr[x_{tj}|C_k]
\end{equation}

In our problem, for each training data $x_i$, $x_{ij}$ is independently perturbed by randomized response at $O_i$ and $x_i'$ is sent to the Data User. The Data User fits the Naive Bayes classifier using $x_i',y_i, i=1,2,\dots,n$. To calculate $Pr[x_{tj}=v|C_k]$, the frequency of value $v$ in the $j$th feature that belongs to $C_k$ should be counted, in which is denoted as $c_j(v)$. However, due to the randomized response, the observation doesn't reflect the true proportion of value $v$. Thus given the number of observation of $v$ in the $j$th feature, denoted as $\sum_jv$, $c_j(v)$ is estimated as\cite{wang2017locally}:

\begin{align}
\hat{c_j(v)} & = \frac{\sum_jv - nq_j}{p_j-q_j} \\
& = \frac{\sum_jv - n(1-p_j)/(d-1)}{p_j-(1-p_j)/(d-1)}
\end{align}

where $p_j=Pr[x_{ij}'=v]$, if $x_{ij}=v$, which refers to Equ.\ref{equ:randmizedResponse}, and $n$ is the number of observations that in $C_k$. It can be further shown that $\hat{c_j(v)}$ is an unbiased estimator. Assuming $f_{v,j}$ is the true proportion that value $v$ occurs in $j$th feature, $E[\hat{c_j(v)}]$ would be:

\begin{align}
E[\hat{c_j(v)}] & = E[\frac{\sum_jv - nq_j}{p_j-q_j}] \\
& = \frac{nf_{v,j}p_j+n(1-f_{v,j})q_j-nq_j}{p_j-q_j} \\ 
& = nf_{v,j}
\end{align}

And $Var[\hat{c_j(v)}]$ is given by:
\begin{align}
Var[\hat{c_j(v)}] & = \frac{nq_j(1-q_j)}{(p_j-q_j)^2} + \frac{nf_{v,j} (1-p_j-q_j)}{p_j-q_j} \\
& = n(\frac{d-2+e^{\epsilon_j}}{(e^{\epsilon_j}-1)^2} + \frac{f_{v,j}(d-2)}{e^{\epsilon_j}-1})
\end{align}

With the unbiased estimator of $c_j(v)$, $Pr[x_{tj} = v|C_k]$ is calculated as:
\begin{equation}
Pr[x_{tj}=v|C_k] = \frac{\hat{c_j(v)}}{\hat{c_1(v)}+\hat{c_2(v)}+\dots+\hat{c_d(v)}}
\end{equation}

It is readily to see that the utility of the Naive Bayes classifier is determined by $\hat{c_j(v)}$, where $Var[\hat{c_j(v)}]$ indicates that the estimation error is in $O(nd)$. Since there are $m$ features in total and Naive Bayes assumes that features are independent, the total estimation error is in $O(mnd)$. When $n$ and $m$ is fixed, the larger $d$ is, the bigger $Var[\hat{c_j(v)}]$ is. Thus the utility of the Naive Bayes classifier is linearly dependent on the domain size. 


\subsubsection{Distance between Perturbed Data Points}
In KNN algorithm, the testing data is classified based on the majority votes of its $k$ nearest training data. Instead of estimating the frequency of each value occurred in the input, the utility of the KNN classifier relies on the noisy input themselves, where the utility can be maintained as long as the proximity of the perturbed input remains the same. To illustrate the statement, we analyze the $p$-norm distance between the testing data and the perturbed training data. 

Given the training data $x_i=[x_{i1},x_{i2},\dots,x_{im}]^T$ before perturbation and $x_i'=[x_{i1}',x_{i2}',\dots,x_{im}']^T$ after perturbation. For $x_{ij}$, $p_{ij}=Pr[x_{ij}=x_{ij}']=\frac{e^\epsilon}{d-1+e^\epsilon}$ and $q_{ij}=Pr[x_{ij}\neq x_{ij}']= \frac{1-p}{d-1} = \frac{1}{d-1+e^\epsilon}$, where $d\geq2$. The $p$-norm distance between two data points $x_i$ and $x_j$ is defined as $\ell_p(x_i,x_j) = (\sum_{k=1}^m(|x_{ik}-x_{jk}|)^p)^{1/p}$. Given a testing data $x_t\in {\Bbb Z}^m$, then $E[\ell_p(x_i',x_t)]$ reflects the expected $p$-norm distance between $x_i'$ and $x_t$. As an example, $E[\ell_1(x_i',x_t)]$ is shown below:

\begin{align}
E[\ell_1(x_i',x_t)]
 = & E[\sum_{k=1}^m|x_{ik}'-x_{tk}|]\\
                 =& \sum_{k=1}^m E[|x_{ik}'-x_{tk}|]\\
                 =& \sum_{k=1}^m [p|x_{ik}-x_{tk}|+ q\sum_{x_{ik}\neq x_{ik}'}|x_{ik}'-x_{tk}|]\\
                 =& \sum_{k=1}^m [p|x_{ik}-x_{tk}|+ q\sum_{x_{ik}\neq x_{ik}'}|x_{ik}'-x_{tk}|\\
                 &+q|x_{ik}-x_{tk}| - q|x_{ik}-x_{tk}|]\\
                 =& \sum_{k=1}^m[(p-q)|x_{ik}-x_{tk}|+q\sum_{v=1}^d|v-x_{tk}|]\\
                 =& (p-q)\ell_1(x_i,x_t)+q\sum_{k=1}^m\sum_{v=1}^d|v-x_{tk}|
\end{align}

Additionally, $E[\ell_2(x_i',x_t)]$ follows a similar manner, for ease of computation, we show $E[\ell_2^2(x_i',x_t)]$ as below:
\begin{align}
E[\ell_2^2(x_i',x_t)]
                 =& \sum_{k=1}^m E[(x_{ik}'-x_{tk})^2]\\
                 =& \sum_{k=1}^m [p(x_{ik}-x_{tk})^2+ q\sum_{x_{ik}\neq x_{ik}'}(x_{ik}'-x_{tk})^2]\\
                 =& \sum_{k=1}^m [p(x_{ik}-x_{tk})^2+ q\sum_{x_{ik}\neq x_{ik}'}(x_{ik}'-x_{tk})^2\\
                 &+q(x_{ik}-x_{tk})^2 - q(x_{ik}-x_{tk})^2]\\
                 =& (p-q)\ell_2^2(x_i,x_t)+q\sum_{k=1}^m\sum_{v=1}^d(v-x_{tk})^2
\end{align}
Thus, with two perturbed training data $x_i',x_j'$ and the testing data $x_t$, the proximity of the expected distance can be expressed as:
\begin{equation}
E[\ell_2^2(x_j',x_t)] = (p-q)\ell_2^2(x_j,x_t)+q\sum_{k=1}^m\sum_{v=1}^d(v-x_{tk})^2
\end{equation}

\begin{align}
E[\ell_2^2(x_i',x_t)-\ell_2^2(x_j',x_t)] =& E[\ell_2^2(x_i',x_t)]-E[\ell_2^2(x_j',x_t)] \\
=& (p-q)(\ell_2^2(x_i,x_t)-\ell_2^2(x_j,x_t))\\
=& \frac{e^\epsilon-1}{d-1+e^\epsilon}(\ell_2^2(x_i,x_t)-\ell_2^2(x_j,x_t))
\end{align}
where $0\leq \frac{e^\epsilon-1}{d-1+e^\epsilon} < 1$ and it entails the probability of being the true difference of the noise-free distances. With a specified privacy level, i.e. a fixed $\epsilon$, the probability is inversely proportional to $d$, and $\frac{e^\epsilon-1}{d-1+e^\epsilon} \approx \frac{1}{2}$ when $\epsilon \approx ln(d+1)$. The setting $\epsilon \approx ln(d+1)$ implies that the probability of preserving the true proximity is $\frac{1}{2}$ and lying uniformly over the remainder of domain $[d]$ with probability $\frac{1}{2}$, which reflects a reasonably notion of plausible deniability. Empirically, our experiments also show that the classification accuracy is almost compatible to the non-perturbed input when $\epsilon \geq ln(d+1)$.
